Fast and Interpretable Mortality Risk Scores for Critical Care Patients

Prediction of mortality in intensive care unit (ICU) patients typically relies on black box models (that are unacceptable for use in hospitals) or hand-tuned interpretable models (that might lead to the loss in performance). We aim to bridge the gap between these two categories by building on modern interpretable ML techniques to design interpretable mortality risk scores that are as accurate as black boxes. We developed a new algorithm, GroupFasterRisk, which has several important benefits: it uses both hard and soft direct sparsity regularization, it incorporates group sparsity to allow more cohesive models, it allows for monotonicity constraint to include domain knowledge, and it produces many equally-good models, which allows domain experts to choose among them. For evaluation, we leveraged the largest existing public ICU monitoring datasets (MIMIC III and eICU). Models produced by GroupFasterRisk outperformed OASIS and SAPS II scores and performed similarly to APACHE IV/IVa while using at most a third of the parameters. For patients with sepsis/septicemia, acute myocardial infarction, heart failure, and acute kidney failure, GroupFasterRisk models outperformed OASIS and SOFA. Finally, different mortality prediction ML approaches performed better based on variables selected by GroupFasterRisk as compared to OASIS variables. GroupFasterRisk's models performed better than risk scores currently used in hospitals, and on par with black box ML models, while being orders of magnitude sparser. Because GroupFasterRisk produces a variety of risk scores, it allows design flexibility - the key enabler of practical model creation. GroupFasterRisk is a fast, accessible, and flexible procedure that allows learning a diverse set of sparse risk scores for mortality prediction.

==> data.tex <==
In our study, we consider Medical Information Mart for Intensive Care III Database (MIMIC-III)\footnote{\href{https://mimic.mit.edu/}{https://mimic.mit.edu/}} and eICU Collaborative Research Database (eICU)\footnote{\href{https://eicu-crd.mit.edu/}{https://eicu-crd.mit.edu/}}\citep{johnson2016mimic, pollard2018eicu}. \footnote{\href{https://eicu-crd.mit.edu/}{https://eicu-crd.mit.edu/}} Our goal is to train high-quality risk scores using \textit{Group FasterRisk} to predict patients' risk of mortality, using only data collected within the first 24 hours of patients' ICU stays. Our models are trained on a subset of MIMIC-III and evaluated on entire eICU dataset.

\subsection*{MIMIC-III} 
MIMIC-III is a large, single-center database comprising health-related information of 53,423 hospital admissions for adult patients (aged 16 years or above) admitted to critical care units of the Beth Israel Deaconess Medical Center in Boston, MA, between 2001 and 2012. MIMIC-III integrates de-identified, comprehensive clinical data of 38,597 distinct adult patients. It includes patient information such as laboratory measurements, vital signs, notes charted by healthcare providers, diagnostic codes, hospital length of stay, and survival data. Besides mortality prediction, MIMIC-III has been used by academic and industrial research to investigate novel clinical relationships and develop new algorithms for patient monitoring \citep*{johnson2016mimic}.

\subsection*{eICU}
The eICU Collaborative Research Database, sourced from the eICU Telehealth Program, is a multi-center ICU database with high granularity data with 200,859 admissions to ICUs monitored by eICU programs across the United States. The database comprises 139,367 unique patients admitted to critical care units in 2014 and 2015. Built upon the success of MIMIC-III, eICU includes patients from multiple medical centers instead of one. The source hospital of MIMIC-III does not participate in the eICU program, which makes eICU a completely independent set of healthcare data suitable for out of distribution evaluation \citep*{pollard2018eicu}.



==> fairness.tex <==


%We also provided the comparative experiment where we calibrate severity of illness score baselines in Supplementary Material \ref{appendix:add exp:fairness calibration}; the results did not change.

% \textbf{Calibration Evaluation Metrics:}
% In mortality risk prediction, even if a model demonstrates high accuracy based on AUROC and AUPRC, it may not provide precise risk probability estimates. This is because they are rank statistics \cite{huang2020tutorial}.
% We evaluate reliability based on \textit{Brier score}, \textit{Hosmer-Lemeshow $\chi^2$ statistics} (HL $\chi^2$), and the \textit{standardized mortality ratio} (SMR) \cite{brier1950verification, lemeshow1982review}.
% We use $C$-statistics for HL $\chi^2$, calculated from deciles of predicted probabilities.
% Unless mentioned otherwise, we use paired $t$-test for statistical testing, and the p-value is denoted with $p$.

% \subsection{\ouralg Produces Reliable and Fair Risk Predictions \label{sec:results:fairness and calibration}}
% % In critical care settings, the trustworthiness and fairness of a model's predictions are paramount since they could considerably affect its usability \cite{mehrabi2021survey}.
% To assess the \ouralg models and the severity of illness score baselines, we use the calibration and predictive accuracy metrics outlined in ``Calibration Metrics'' section in Methods.
% %\Cref{study_overview:setup}.
% We consider our eICU cohort for the evaluations because it offers a larger sample size and encompasses multi-center data from across the United States.
% Subsequently, we evaluate \ouralg models across various demographic subgroups, considering factors like ethnicity and gender.

% Our results are presented in \Cref{fairness and calibration}.
% We observe that \ouralg models are not particularly biased towards the majority race (Caucasians) and are well-calibrated on specific subgroups in our eICU cohort.
% % \ouralg models consistently achieve low Brier scores and HL $\chi^2$ across population subgroups.
% % Except in a few cases, \ouralg models' Brier scores, HL $\chi^2$, and SMR are better than those of OASIS, SAPS II, and APACHE IV/IVa.
% % On average, across all ethnic and gender groups, GFR-10, GFR-15, and GFR-40 achieve SMR of 0.986$\pm$0.041, 1.004$\pm$0.040, and 1.005$\pm$0.058, respectively, which are all close to 1 (the best possible value).
% % Among sparse models (no more than 17 variables), \ouralg achieves the highest AUROC and AUPRC across subgroups.
% % We present additional ROC, PR, and calibration curves in \Cref{appendix:add exp:fairness calibration}.



==> other.tex <==
\subsection*{Code Availability} 
\todolist{Final Git Repo?}
All the code written to extract features from MIMIC-III and eICU and produce the experiments of this paper is made freely available on ?. Furthermore, the MIT Laboratory of Computational Physiology (MIT-LCP) curates two repositories containing code written for all MIMIC and eICU databases.

\subsection*{Data Availability}
Both the MIMIC-III and eICU datasets are produced by researchers from the MIT Laboratory for Computation Physiology (MIT-LCP). Other researchers can access the underlying data used to produce our results by registering for access on the PhysioNet platform. This request requires two principal components:

\begin{itemize}
    \item Completed a recognized course in protecting human research participants that covers Health Insurance Portability and Accountability Act (HIPAA). 
    \item Signed a data use agreement outlining appropriate data usage and security standards and forbids any efforts to identify individual patients. 
\end{itemize}

Once this request is granted, the databases can be accessed either through Cloud platforms or downloaded locally. Full instructions for both the MIMIC-III and eICU  platforms can be found on their respective websites. \footnote{See https://mimic.mit.edu/docs/gettingstarted/ and https://eicu-crd.mit.edu/gettingstarted/access/}.
